MUSE Analysis of Gas around Galaxies (MAGG) -- VI. The cool and enriched gas environment of z$\gtrsim$3 Ly$\alpha$ emitters

We present a novel dataset that extends our view of the cosmic gas around z$\approx$3-4 Ly$\alpha$ emitting galaxies (LAEs) in the Muse Analysis of Gas around Galaxies (MAGG) survey by tracing a cool and enriched gas phase through 47 MgII absorbers identified in newly-obtained VLT/XSHOOTER near-infrared quasar spectra. Jointly with the more ionized gas traced by CIV systems and the neutral HI from previous work, we find that LAEs are distributed inside cosmic structures that contain multiphase gas in composition and temperature. All gas phases are a strong function of the large-scale galaxy environment: the MgII and the CIV strength and kinematics positively correlate with the number of associated galaxies, and it is $\approx$3-4 times more likely to detect metal absorbers around group than isolated LAEs. Exploring the redshift evolution, the covering factor of MgII around group and isolated LAEs remains approximately constant from z$\approx$3-4 to z<2, but the one of CIV around group galaxies drops by z<2. Adding the cool enriched gas traced by the MgII absorbers to the results we obtained for the HI and CIV gas, we put forward a picture in which LAEs lie along gas filaments that contain high column-density HI systems and are enriched by strong CIV and MgII absorbers. While the MgII gas appears to be more centrally concentrated near LAEs, weaker CIV systems trace instead a more diffuse gas phase extended up to larger distances around the galaxies.

==> NOTES.tex <==

% LF and xCorr for CIV with EW >= 0.10 A
Given the different selection function for the MgII and CIV samples, one option is to consider only the strong CIV absorbers. At the moment I am taking the CIV absorbers with EW > 0.10 A (99 CIV absorbers out of 220), corresponding to the completeness limit of the MgII in the NIR. This is what happens to the CIV LF.

\begin{equation}
\begin{split}
    \log[\phi^\star/({\rm Mpc^{-3}dex^{-1}})]=-1.817\pm 0.307 \\
    \log[{L}^\star/({\rm erg\,s^{-1}})]=42.476\pm 0.218 \\
    \alpha=-1.234\pm 0.399  
\end{split}
\end{equation}

Rough results coming straight from the MCMC fit.
Best alpha = -1.234254960226905 pm 0.39919294193479593
Best Lstar = 42.47602364043007 pm 0.21792613246104509
Best phist = 0.01516698051533179
Phi to use:  [-2.20478612 -1.817218 -1.5911019]

With the same motivation we can also check what changes in the cross-correlation function when only this population of CIV is taken into account. We measure again R0 assuming EW>= 0.1 A for the CIV. Expected density for a field/random sample: $N_{\rm LAEs}/{\rm Area}=16.157^{4.873}_{4.153}\,h^{2}Mpc^{-2}$. Correlation length: $\gamma=1.8$ $r_{0}=1.400^{+0.325}_{-0.408}\,h^{-1}Mpc$.

% Abstract
We present a study of the multiphase gas around Ly$\alpha$ emitting galaxies in the Muse Analysis of Gas around Galaxies (MAGG) survey at $z\approx3-4$. We trace a cool and enriched gas phase via 47 \mgii\ absorbers identified in new VLT/XSHOOTER near-infrared quasar spectra, recently integrated in MAGG. Jointly to the warmer and more ionized gas traced by \civ\ systems presented in \maggv, we simultaneously investigate the properties of the different gas phases and compare their link to the galaxies. This is found be a strong function of the large-scale galaxy environment. Indeed, both the \mgii\ and the \civ\ strength and kinematics positively correlate with the number of associated galaxies. We observe that detecting metal absorbers around groups is $\approx2-3$ times more likely than around isolated LAEs, regardless the gas phase. While the abundance of \mgii\ around groups and isolated LAEs remains approximately constant from $z\approx3.4$ down to $z\lesssim2$, that of \civ\ around galaxies in groups drops significantly by $z\lesssim2$. We propose a scenario in which this effect is due to the different distribution of the gas phases around galaxies: the \civ\ is more extended than the \mgii\ gas and thus likely ionized to higher stages in overdense environments at lower redshifts.

% (Sub)Section on detection rates - 4.1.1
\subsubsection{Rates of gas-galaxy connections}

\begin{figure} 
\centering
\includegraphics[width=\columnwidth]{Detection_rate_details_clean.pdf}
\caption{Fraction of \mgii\ (orange) and \civ\ (black) absorbers with equivalent width $W_{\rm r}\geq W_0$ that are found to be connected to at least one LAE within $\pm500\rm\,km\,s^{-1}$ as a function of the threshold $W_0$.}
\label{fig:det_rate}
\end{figure}

The rate at which we are able to find one or more galaxies close in velocity to the absorbers provides information about which type of galaxies are surrounded by different gas phases. We thus estimate the fraction of $W_{\rm r}\geq W_0$ absorbers that are connected to at least one LAE within $\pm500\rm\,km\,s^{-1}$, as a function of their rest-frame equivalent width. As shown in Figure \ref{fig:det_rate}, the detection rate increases monotonically with the strength of the \civ\ absorbers (black). Instead, we do not find any significant trend for the cooler \mgii\ gas (orange). The Spearman-rank correlation test results in $\rho=0.99$, $p-$value$=0.003$ for the \civ\ and $\rho=-0.26$, $p-$value$=0.63$ for the \mgii\ gas, supporting these conclusions. In order to further explore this difference, we focus on the strong $W_{\rm r}^{\rm\mgii}\geq1\,\text{\AA}$ \mgii\ absorbers as well as on the \civ\ systems that are found to be aligned with the cool gas in redshift space (see the Appendix \ref{app:kinematics}). We observe that the presence of at least one LAE correlates with a separation in the \civ\ equivalent width, with $W_{\rm r}^{\rm\civ}\lesssim0.6\text\,{\AA}$ (corresponding to the 95th percentile of the \civ\ equivalent width distribution) systems not being connected to any galaxy, while stronger \civ\ are. Altogether, the weakness of the \civ\ absorbers and the strength of the \mgii\ systems suggests either an excess of cool gas or a lower ionization. A galaxy population different from the one that we targeted, thus excluded from our selection, e.g. dusty-obscured galaxies, may be connected to these strong cool systems. \citet{Menard2015} studied the dust content of strong $W_{\rm r}\geq0.8\,\text{\AA}$ \mgii\ absorbers. At $z\approx0.5$, they found that it is similar to the dust content of galactic disks and showed that the \mgii\ absorbers carry $\approz1/2-1/3$ of the total dust expelled by galaxies. Similarly, \citet{Budzynski2011} reported that in SDSS the $\approx20\%$ of $W_{\rm r}\geq1\,\text{\AA}$ \mgii\ systems are missed due to heavy dust obscuration. If on one hand this compilation of studies suggests that the gaseous environment in which the strong \mgii\ systems reside is rich in dust, the lack of infrared observations prevent us from drawing any robust conclusion. 

As a final step, we explore the possibility that the galaxies connected to these strong absorbers lie at close separation from the sightline \citep[see e.g.][]{}. We thus project 14 layers around the wavelength of the Ly$\alpha$ emission at the redshift of the absorbers to build pseudo-narrow band cut-outs around the central quasar of each field from the continuum-subtracted datacubes. By visually inspecting these images, we did not find any Ly$\alpha$ emitting galaxies that was not identified by our selection due to their proximity or overlap with the quasar point-spread-function. 

A larger sample of strong absorbers as well as higher resolution and IR observations for the galaxies would be instrumental to test whether the presence of galaxies closer than $\approx0.8\rm\,arcsec$ to the sightline, a different population or the combination of these two scenarios may be responsible for the observed detection rate around the strongest \mgii\ absorbers.





